Hierarchical Gradient-Based Genetic Sampling for Accurate Prediction of Biological Oscillations

Biological oscillations are periodic changes in various signaling processes crucial for the proper functioning of living organisms. These oscillations are modeled by ordinary differential equations, with coefficient variations leading to diverse periodic behaviors, typically measured by oscillatory frequencies. This paper explores sampling techniques for neural networks to model the relationship between system coefficients and oscillatory frequency. However, the scarcity of oscillations in the vast coefficient space results in many samples exhibiting non-periodic behaviors, and small coefficient changes near oscillation boundaries can significantly alter oscillatory properties. This leads to non-oscillatory bias and boundary sensitivity, making accurate predictions difficult. While existing importance and uncertainty sampling approaches partially mitigate these challenges, they either fail to resolve the sensitivity problem or result in redundant sampling. To address these limitations, we propose the Hierarchical Gradient-based Genetic Sampling (HGGS) framework, which improves the accuracy of neural network predictions for biological oscillations. The first layer, Gradient-based Filtering, extracts sensitive oscillation boundaries and removes redundant non-oscillatory samples, creating a balanced coarse dataset. The second layer, Multigrid Genetic Sampling, utilizes residual information to refine these boundaries and explore new high-residual regions, increasing data diversity for model training. Experimental results demonstrate that HGGS outperforms seven comparative sampling methods across four biological systems, highlighting its effectiveness in enhancing sampling and prediction accuracy.

==> ReproducibilityChecklist.tex <==
\section{Reproducibility Checklist}
\paragraph{This paper:}
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) {\textbf{yes}}
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) {\textbf{yes}}
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) {\textbf{yes}}
\end{itemize}

\paragraph{Does this paper make theoretical contributions? (yes/no) {\textbf{no}}}
If yes, please complete the list below.
\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
\item Proofs of all novel claims are included. (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\paragraph{Does this paper rely on one or more datasets? (yes/no) {\textbf{yes}}}
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) {\textbf{yes}}
\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) {\textbf{yes}}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) {\textbf{yes}}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) {\textbf{yes}}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) {\textbf{yes}}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) {\textbf{yes}}
\end{itemize}

\paragraph{Does this paper include computational experiments? (yes/no) {\textbf{yes}}}
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes/partial/no). {\textbf{yes}}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) {\textbf{yes}}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) {\textbf{yes}}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) {\textbf{yes}}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) {\textbf{yes}}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) {\textbf{yes}}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) {\textbf{yes}}
\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) {\textbf{yes}}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) {\textbf{yes}}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) {\textbf{no}}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) {\textbf{yes}}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) {\textbf{yes}}
\end{itemize}

